Closure hyperdoctrines, with paths

(Pre)closure spaces are a generalization of topological spaces covering also the notion of neighbourhood in discrete structures, widely used to model and reason about spatial aspects of distributed systems. In this paper we introduce an abstract theoretical framework for the systematic investigation of the logical aspects of closure spaces. To this end, we introduce the notion of closure (hyper)doctrines, i.e. doctrines endowed with inflationary operators (and subject to suitable conditions). The generality and effectiveness of this concept is witnessed by many examples arising naturally from topological spaces, fuzzy sets, algebraic structures, coalgebras, and covering at once also known cases such as Kripke frames and probabilistic frames (i.e., Markov chains). Then, we show how spatial logical constructs concerning surroundedness and reachability can be interpreted by endowing hyperdoctrines with a general notion of paths. By leveraging general categorical constructions, we provide axiomatisations and sound and complete semantics for various fragments of logics for closure operators. Therefore, closure hyperdoctrines are useful both for refining and improving the theory of existing spatial logics, but especially for the definition of new spatial logics for new applications.

==> pratenddefaultcategory.tex <==

\label{proofsection:prAtEndii}\begin{proof}[Proof of \autoref{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}We have to show that $\mathscr {P}_{\mathscr {F}(\pi _D)}$ has a left adjoint for any projection $\pi _D:E\times D\rightarrow D$ but this follows at once since the horizontal arrow in the diagram \begin {center} \begin {tikzpicture} \node (F)at(0,0){$\mathscr {P}(\mathscr {F}(E\times D))$}; \node (I)at(6,0){$\mathscr {P}(\mathscr {F}(E)\times \mathscr {F}(D))$}; \node (G)at(3,2){$\mathscr {P}(\mathscr {F}(D))$}; \draw [<-](F)--(G)node[pos=0.5, above, xshift=-0.4cm]{$\mathscr {P}_{\mathscr {F}(\pi _D)}$}; \draw [<-](I)--(G)node[pos=0.5, above, xshift=0.2cm, yshift=-0.05cm]{$\mathscr {P}_{\pi _{\mathscr {F}(D)}}$}; \draw [<-](I)--(F)node[pos=0.5,below]{$\mathscr {P}_{(\mathscr {F}(\pi _E),\mathscr {F}(\pi _D))}$}; \end {tikzpicture} \end {center} is an isomorphism, hence \begin {equation*} \exists _{\pi _D}=\exists _{\pi _{\mathscr {F}(D)}}\circ \mathscr {P}_{(\mathscr {F}(\pi _E),\mathscr {F}(\pi _D))} \end {equation*} The same argument shows the existence of right adjoint to $\mathscr {P}_{\mathscr {F}(\pi _D)}$ anytime they exist for $\mathscr {P}_{\pi _{\mathscr {F}(D)}}$: \begin {equation*} \forall _{\pi _D}=\forall _{\pi _{\mathscr {F}(D)}}\circ \mathscr {P}_{(\mathscr {F}(\pi _E),\mathscr {F}(\pi _D))} \end {equation*} Let $f:D'\rightarrow D$ be an arrow in $\catname {D}$, the two Beck-Chevalley conditions follow from the commutativity of \begin {center} \begin {tikzpicture} \node (F)at(0,2){$\mathscr {P}(\mathscr {F}(E\times D))$}; \node (I)at(0,0){$\mathscr {P}(\mathscr {F}(E)\times \mathscr {F}(D))$}; \node (G)at(6,0){$\mathscr {P}(\mathscr {F}(D))$}; \par \node (F')at(0,-4){$\mathscr {P}(\mathscr {F}(E\times D'))$}; \node (I')at(0,-2){$\mathscr {P}(\mathscr {F}(E)\times \mathscr {F}(D'))$}; \node (G')at(6,-2){$\mathscr {P}(\mathscr {F}(D'))$}; \draw [<-](F)..controls(4,1.5)..(G)node[pos=0.5, above, yshift=0cm]{$\mathscr {P}_{\mathscr {F}(\pi _D)}$}; \draw [<-](I)--(G)node[pos=0.5, above, xshift=0cm, yshift=0cm]{$\mathscr {P}_{\pi _{\mathscr {F}(D)}}$}; \draw [<-](I)--(F)node[pos=0.5, right]{$\mathscr {P}_{(\mathscr {F}(\pi _E),\mathscr {F}(\pi _D))}$}; \par \par \draw [<-](F')..controls(4,-3.5)..(G')node[pos=0.5, below, yshift=-0.1cm]{$\mathscr {P}_{\mathscr {F}(\pi _{D'})}$}; \draw [<-](I')--(G')node[pos=0.5, below]{$\mathscr {P}_{\pi _{\mathscr {F}(D')}}$}; \draw [<-](I')--(F')node[pos=0.5,right]{$\mathscr {P}_{(\mathscr {F}(\pi _E),\mathscr {F}(\pi _D))}$}; \par \draw [<-](G)--(G')node[pos=0.5,right]{$\mathscr {P}_{\mathscr {F}(f)}$}; \draw [<-](I)--(I')node[pos=0.5,left]{$\mathscr {P}_{1_{\mathscr {F}(E)}\times \mathscr {F}(f)}$}; \draw [->](F')..controls(-3,-4) and (-3, 2)..(F)node[pos=0.5,left]{$\mathscr {P}_{\mathscr {F}(1_E\times f)}$}; \end {tikzpicture} \end {center} and the fact that both the upper and the lower vertical arrow are isomorphisms since $\mathscr {F}$ preserves products. For Frobenius reciprocity: \begin {align*} \exists _{\mathscr {F}(\pi _D)}(\mathscr {P}_{\mathscr {F}(\pi _D)}(\alpha )\wedge \beta )&= \exists _{\pi _{\mathscr {F}(D)}}(\mathscr {P}_{(\mathscr {F}(\pi _E),\mathscr {F}(\pi _D))}(\mathscr {P}_{\mathscr {F}(\pi _D)}(\alpha )\wedge \beta ))\\&= \exists _{\pi _{\mathscr {F}(D)}}(\mathscr {P}_{\pi _{\mathscr {F}(D)}}(\alpha )\wedge \mathscr {P}_{(\mathscr {F}(\pi _E),\mathscr {F}(\pi _D))}(\beta ))\\&=\alpha \wedge \exists _{\pi _{\mathscr {F}(D)}}(\mathscr {P}_{\mathscr {F}(\pi _D)}(\alpha )\wedge \beta )\\&= \alpha \wedge \exists _{\mathscr {F}(\pi _D)}(\beta ) \end {align*} So we're left with the fibered equalities, by the commutativity of \begin {center} \begin {tikzpicture} \node (A) at(0,2) {$\mathscr {P}(\mathscr {F}(E\times D \times D))$}; \node (C) at(8,2) {$\mathscr {P}(\mathscr {F}(E)\times \mathscr {F}(D) \times \mathscr {F}(D))$}; \node (B) at(0,0) {$\mathscr {P}(\mathscr {F}(E\times D))$}; \node (D) at(8,0) {$\mathscr {P}(\mathscr {F}(E)\times \mathscr {F}(D))$}; \draw [->] (A)--(B) node[pos=0.5, left]{$\mathscr {P}_{\mathscr {F}(1_E\times \Delta _D)}$}; \draw [<-] (A)--(C) node[pos=0.5, above]{$\mathscr {P}_{(\mathscr {F}(\pi _1),\mathscr {F}(\pi _2),\mathscr {F}(\pi _3))}$}; \draw [->] (C)--(D) node[pos=0.5, right]{$\mathscr {P}_{1_{\mathscr {F}(E)}\times \Delta _{\mathscr {F}(D)}}$}; \draw [<-] (B)--(D) node[pos=0.5, below]{$\mathscr {P}_{(\mathscr {F}(\pi _E), \mathscr {F}(\pi _D))}$}; \par \node (B') at(0,-2) {$\mathscr {P}(\mathscr {F}(D\times D))$}; \node (D') at(8,-2) {$\mathscr {P}(\mathscr {F}(D)\times \mathscr {F}(D))$}; \node (A) at(0,-4) {$\mathscr {P}(\mathscr {F}(E\times D \times D))$}; \node (C) at(8,-4) {$\mathscr {P}(\mathscr {F}(E)\times \mathscr {F}(D) \times \mathscr {F}(D))$}; \node (B) at(0,-6) {$\mathscr {P}(\mathscr {F}(E\times D))$}; \node (D) at(8,-6) {$\mathscr {P}(\mathscr {F}(E)\times \mathscr {F}(D))$}; \draw [<-] (A)--(B) node[pos=0.5, left]{$\mathscr {P}_{\mathscr {F}(\pi _1, \pi _2)}$}; \draw [<-] (A)--(B') node[pos=0.5, left]{$\mathscr {P}_{\mathscr {F}(\pi _2, \pi _3)}$}; \draw [<-] (A)--(C) node[pos=0.5, above]{$\mathscr {P}_{(\mathscr {F}(\pi _1),\mathscr {F}(\pi _2),\mathscr {F}(\pi _3))}$}; \draw [<-] (C)--(D) node[pos=0.5, right]{$\mathscr {P}_{(\mathscr {F}(\pi _1),\mathscr {F}(\pi _2))}$}; \draw [<-] (C)--(D') node[pos=0.5, right]{$\mathscr {P}_{(\mathscr {F}(\pi _2),\mathscr {F}(\pi _3))}$}; \draw [<-] (B)--(D) node[pos=0.5, below]{$\mathscr {P}_{(\mathscr {F}(\pi _E), \mathscr {F}(\pi _D))}$}; \draw [<-] (B')--(D') node[pos=0.5, above]{$\mathscr {P}_{(\mathscr {F}(p_1), \mathscr {F}(p_2))}$}; \par \par \par \end {tikzpicture} \end {center} and from the fact that the horizontal arrows are isomorphisms it is enough to take \begin {equation*} \delta _D:=\mathscr {P}_{(\mathscr {F}(p_1), \mathscr {F}(p_2))}(\delta _{\mathscr {F}(D)}) \end {equation*}\qedhere \end{proof}
\label{proofsection:prAtEndiii}\begin{proof}[Proof of \autoref{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}(Cfr. \cite {jacobs1999categorical,lawvere1970equality} and lemma $1.5.8$ of \cite {johnstone2002sketches}, vol. $1$ for the hyperdoctrine case). It is enough to define \begin {align*} \exists _f(\alpha )&:= \exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _C}(\alpha ) ) \\\forall _f(\alpha )&:= \forall _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D)\rightarrow \mathscr {P}_{\pi _C}(\alpha ) ) \end {align*} For adjointness: \begin {itemize} \item $\exists _f \dashv \mathscr {P}_f$. \begin {equation*} \begin {split} \text {If} \ \exists _f(\alpha )&\leq \beta \\ \alpha &= \alpha \wedge \top _C \\ &= \alpha \wedge \exists _{\pi _2}(\delta _C)\\ &\leq \alpha \wedge \exists _{\pi _2}(\mathscr {P}_{f\times f}(\delta _D))\\ &= \exists _{\pi _2}(\mathscr {P}_{f\times f}(\delta _D)\wedge \mathscr {P}_{p_2}(\alpha ))\\ &=\exists _{\pi _2}(\mathscr {P}_{1_C\times f}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _C}(\alpha ))\\ &=\mathscr {P}_f(\exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _C}(\alpha ) ))\\ &=\mathscr {P}_f(\exists _f(\alpha ))\\ &\leq \mathscr {P}_f(\beta )\\ & \end {split} \begin {split} \text {If} \ \alpha &\leq \mathscr {P}_f(\beta )\\ \exists _f(\alpha )&\leq \exists _f(\mathscr {P}_f(\beta ))\\&= \exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _C}(\mathscr {P}_f(\beta ) )\\&=\exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{1_D\times f}(\mathscr {P}_{q_2}(\beta ) ))\\&= \exists _{\pi _D}(\mathscr {P}_{ 1_D\times f}(\delta _D)\wedge \mathscr {P}_{1_D\times f}(\mathscr {P}_{q_2}(\beta ) )) \\&= \exists _{\pi _D}(\mathscr {P}_{ 1_D\times f}(\delta _D\wedge \mathscr {P}_{q_2}(\beta ))) \\&=\exists _{\pi _D}(\mathscr {P}_{ 1_D\times f}(\exists _{\Delta _D}(\beta )))\\&\leq \exists _{\pi _D}(\mathscr {P}_{ 1_D\times f}(\mathscr {P}_{q_1}(\beta )))\\&=\exists _{\pi _D}(\mathscr {P}_{\pi _D}(\beta ))\\&\leq \beta \end {split} \end {equation*} Where $p_2$ is the second projection $C\times C\rightarrow C$ and $q_1$ and $q_2$ those $D\times D\rightarrow D$. \item $\mathscr {P}_f\dashv \forall _f$. We already know that: \begin {equation*} \exists _{\pi _C}\dashv \mathscr {P}_{\pi _C} \quad \mathscr {P}_{f\times 1_D}(\delta _D)\wedge (-) \dashv \mathscr {P}_{f\times 1_D}(\delta _D)\rightarrow (-) \quad \mathscr {P}_{\pi _D}\dashv \forall _{\pi _D} \end {equation*} so it is enough to show, for all $\beta \in \mathscr {P}(D)$ \begin {equation*} \mathscr {P}_f(\beta ) = \exists _{\pi _C}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _D}(\beta )) \end {equation*} but this is easily done: \begin {align*} \exists _{\pi _C}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _D}(\beta ))&= \exists _{\pi _C}(\mathscr {P}_{1_D\times f}(\delta _D)\wedge \mathscr {P}_{1_D\times f}(\mathscr {P}_{\pi _1}(\beta )))\\&= \exists _{\pi _C}(\mathscr {P}_{1_D\times f}(\delta _D\wedge \mathscr {P}_{\pi _1}(\beta )))\\&= \mathscr {P}_f(\exists _{\pi _2}(\exists _{\Delta _D}(\beta )))\\&=\mathscr {P}_f(\beta ) \end {align*} Where $\pi _2$ is the second projection $D\times D\rightarrow D$. \end {itemize} For Frobenius reciprocity: the inequality $ \exists _{f}(\mathscr {P}_{f}(\beta )\wedge \alpha )\leq \beta \wedge \exists _{f}(\alpha )$ follows from adjointness, let's show the other. Let $\pi _1$ and $\pi _2$ be the projections from $D\times D$ and compute: \begin {align*} \exists _{f}(\mathscr {P}_{f}(\beta )\wedge \alpha )&= \exists _{\pi _D}(\mathscr {P}_{f \times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _C}(\mathscr {P}_f(\beta )\wedge \alpha ))\\&=\exists _{\pi _D}(\mathscr {P}_{f \times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _C}(\mathscr {P}_f(\beta ))\wedge \mathscr {P}_{\pi _C}(\alpha ))\\&= \exists _{\pi _D}(\mathscr {P}_{f \times 1_D}(\delta _D)\wedge \mathscr {P}_{f\times 1_D}(\mathscr {P}_{\pi _1}(\beta ))\wedge \mathscr {P}_{\pi _C}(\alpha ))\\&= \exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D\wedge \mathscr {P}_{\pi _1}(\beta )) \wedge \mathscr {P}_{\pi _C}(\alpha ))\\&\leq \exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D\wedge \mathscr {P}_{\pi _2}(\beta )) \wedge \mathscr {P}_{\pi _C}(\alpha ))\\&= \exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{f\times 1_D}(\mathscr {P}_{\pi _2}(\beta )) \wedge \mathscr {P}_{\pi _C}(\alpha ))\\&= \exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D)\wedge \mathscr {P}_{\pi _D}(\beta ) \wedge \mathscr {P}_{\pi _C}(\alpha ))\\&=\exists _{\pi _D}(\mathscr {P}_{f\times 1_D}(\delta _D) \wedge \mathscr {P}_{\pi _C}(\alpha ))\wedge \beta \\&= \exists _f(\alpha )\wedge \beta \end {align*} where we have used the inequality: \begin {equation*} \delta _D\wedge \mathscr {P}_{\pi _1}(\beta ) \leq \mathscr {P}_{\pi _2}(\beta ) \end {equation*} that follows at once by the definition of $\exists _{\Delta _D}$. \qedhere \end{proof}
\label{proofsection:prAtEndiv}\begin{proof}[Proof of \autoref{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Let's compute: \begin {gather*} \mathfrak {c}_C\circ \mathscr {P}_f \leq \mathscr {P}_f\circ \exists _{f}\circ \mathfrak {c}_C\circ \mathscr {P}_f \leq \mathscr {P}_f \circ \mathfrak {c}_D\circ \exists _{f}\circ \mathscr {P}_f \leq \mathscr {P}_f\circ \mathfrak {c}_D \\ \exists _{f}\circ \mathfrak {c}_C \leq \exists _{f}\circ \mathfrak {c}_C\circ \mathscr {P}_f\circ \exists _{f} \leq \exists _{f}\circ \mathscr {P}_f\circ \mathfrak {c}_D\circ \exists _{f} \leq \mathfrak {c}_D\circ \exists _{f} \qedhere \end {gather*}\end{proof}
\label{proofsection:prAtEndv}\begin{proof}[Proof of \autoref{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}\begin {enumerate} \item For $k$ and $c$ the proposition is obvious, let us examine $\mathfrak {k}$: since $\dot {x}\in q_X(x)$ then $A\subset \mathfrak {k}_X(A)$, if $A\subset B$ then any filters that contains the former contains the latter too and this implies monotonicity, groundedness follows from the fact that $\emptyset $ does not belong to any proper filter, for additivity we can complete any filter $\mathcal {F}$ to which $A\cup B$ belong to an ultrafilter $\mathcal {U}$ that belongs to $q_X(x)$ since the latter is upward closed, either $A$ or $B$ must belong to $\mathscr {U}$ and we are done. \item $\mathscr {i}$ sends a topological space to the pretopological space given by the closure operator associate to its topology, $\mathscr {j}$ sends $(X, \mathfrak {c})$ to $(X,q^{\mathfrak {c}}_X)$ where \begin {align*} q^{\mathfrak {c}}_X:X & \rightarrow \mathcal {P}(\catname {Fil}(X))\\ x & \mapsto \{\mathcal {F}\in \catname {Fil}(X) \mid \mathcal {V}_x\subset \mathcal {F} \} \end {align*} where $\mathcal {V}_x:=\{S \subset X \mid x\notin \mathfrak {c}(X\smallsetminus S)\}$. For the left adjoints see \cite {dikranjan2013categorical}. \item This is obvious.\qedhere \end {enumerate}\end{proof}
\label{proofsection:prAtEndvi}\begin{proof}[Proof of \autoref{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Since the preimage of a normal subgroup is normal we have that the $\nu $ actually exists as a closure operator. The three poperties of it follow immediately by the fact that $\{0\}$ is normal and so are the arbitrary intersections or sums of normal subgroups.\qedhere \end{proof}
\label{proofsection:prAtEndvii}\begin{proof}[Proof of \autoref{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}To show that $\integ {A}(B)$ is a subring of $A$ and idempotency we refer to \cite [Cor.~5.3, 5.5]{atiyah2018introduction}. Let us show that $\integ {}$ is actually a closure operator. Consider $f:A\rightarrow B$ and $C$ a subring of $B$, let $a\in A$ such that $p(a)=0$ for some $p\in f^{-1}(C)[X]$ with coefficients $\{p_i\}_{i=0}^{\deg (p)}$, then $q(f(a))=0$ where $q\in C[X]$ has coefficients $\{f(p_i)\}_{i=0}^{\deg (p)}$ and we are done.\qedhere \end{proof}
\label{proofsection:prAtEndviii}\begin{proof}[Proof of \autoref{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Clearly $f\leq \mathfrak {c}_{X,\epsilon }(f)$ for any $f:X\rightarrow [0,1]$, monotonicity is clear, let's check continuity of any function $g:X\rightarrow Y$: \begin {align*} \mathfrak {c}_{X,\epsilon }(f\circ g)(x) &= (f\circ g)(x)\dot {+}\epsilon \\ &= f(g(x))\dot {+}\epsilon \\ &=\mathfrak {c}_{x,\epsilon }(f)(g(x))\\&=(\mathfrak {c}_{x,\epsilon }(f)\circ g)(x) \qedhere \end {align*}\end{proof}
\label{proofsection:prAtEndix}\begin{proof}[Proof of \autoref{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}We have to show continuity of all arrows $f:(A,\alpha )\rightarrow (B,\beta )$. Let $\xi \in (B,\beta )$ and $x\in A$, we have four cases: \begin {enumerate} \item $f^*(\xi )(x) + \epsilon _{(A,\alpha )}(x)< \alpha (x)$ and $\xi (x) + \epsilon _{(B,\beta )}(x)< \beta (x)$. \begin {align*} (\mathfrak {c}^{\mathscr {E}}_{(A,\alpha )}(f^*(\xi )))(x)&=(f^*(\xi ) + \epsilon _{(A,\alpha )})(x)\\&=(\alpha (x)\wedge \xi (f(x)))+\epsilon _{(A, \alpha )}(x)\\&=\alpha (x)\wedge (\xi (f(x))+\epsilon _{(A, \alpha )}(x))\\&\leq \alpha (x)\wedge (\xi (f(x))+\epsilon _{(B,\beta )}(f(x)))\\&=f^*(\mathfrak {c}^{\mathscr {E}}_{(B,\beta )}(\xi ))(x) \end {align*} \item $f^*(\xi )(x) + \epsilon _{(A,\alpha )}(x)< \alpha (x)$ and $\xi (f(x)) + \epsilon _{(B,\beta )}(f(x))\geq \beta (f(x))$. Notice that $\alpha (x)\leq \beta (f(x))$ so \begin {equation*} f^*(\mathfrak {c}^{\mathscr {E}}_{(B,\beta )}(\xi ))(x)=\alpha (x) \end {equation*} from which: \begin {align*} (\mathfrak {c}^{\mathscr {E}}_{(A,\alpha )}(f^*(\xi )))(x)&=(f^*(\xi ) + \epsilon _{(A,\alpha )})(x)\\&=(\alpha (x)\wedge \xi (f(x)))+\epsilon _{(A, \alpha )}(x)\\&=\alpha (x)\wedge (\xi (f(x))+\epsilon _{(A, \alpha )}(x))\\&=\alpha (x)\\&=f^*(\mathfrak {c}^{\mathscr {E}}_{(B,\beta )}(\xi ))(x) \end {align*} \item $f^*(\xi )(x) + \epsilon _{(A,\alpha )}(x)\geq \alpha (x)$ and $\xi (x) + \epsilon _{(B,\beta )}(x)< \beta (x)$. \begin {align*} (\mathfrak {c}^{\mathscr {E}}_{(A,\alpha )}(f^*(\xi )))(x)&=\alpha (x)\\&=\alpha (x)\wedge (\xi (f(x))+\epsilon _{(A, \alpha )}(x))\\&\leq \alpha (x)\wedge (\xi (f(x))+\epsilon _{(B,\beta )}(f(x)))\\&=f^*(\mathfrak {c}^{\mathscr {E}}_{(B,\beta )}(\xi ))(x) \end {align*} \item $f^*(\xi )(x) + \epsilon _{(A,\alpha )}(x)\geq \alpha (x)$ and $\xi (x) + \epsilon _{(B,\beta )}(x)\geq \beta (x)$. \begin {align*} (\mathfrak {c}^{\mathscr {E}}_{(A,\alpha )}(f^*(\xi )))(x)&=\alpha (x)\\&=\alpha (x)\wedge \beta (f(x))\\&=f^*(\mathfrak {c}^{\mathscr {E}}_{(B,\beta )}(\xi ))(x) \end {align*} We are left with additivity, but this follows immediately since, for $\xi $ and $\zeta \in \fuz (A,\alpha )$ and $x\in A$, $(\xi \vee \zeta )(x)$ is $\xi (x)$ or $\zeta (x)$. \qedhere \end {enumerate}\end{proof}
\label{proofsection:prAtEndx}\begin{proof}[Proof of \autoref{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}\begin {enumerate} \item Clearly $\alpha \leq \diam {X}(\alpha )$; if $\alpha \leq \beta $ we have that \begin {equation*} \mathscr {P}_{\gamma _{X}}(\Box _X(\alpha ))\leq \mathscr {P}_{\gamma _{X}}(\Box _X(\beta )) \end {equation*} from which monotonicity follows; for $f$ an arrow between $\gamma _X:X\rightarrow \mathscr {F}(X)$ and $\gamma _Y:Y\rightarrow \mathscr {F}(Y)$, we have a commutative diagram \begin {center} \begin {tikzpicture} \node (A)at (0,0) {$X$}; \node (B)at (3,0) {$Y$}; \node (C)at (0,-1.5) {$\mathscr {F}(X)$}; \node (D)at (3,-1.5) {$\mathscr {F}(Y)$}; \draw [->](A)--(C) node[pos=0.5, left]{$\gamma _X$}; \draw [->](B)--(D) node[pos=0.5, right]{$\gamma _Y$}; \draw [->](A)--(B) node[pos=0.5, above]{$f$}; \draw [->](C)--(D) node[pos=0.5, below]{$\mathscr {F}(f)$}; \end {tikzpicture} \end {center} and computing we get the thesis: \begin {align*} \diam {X}(\mathscr {P}_f(\alpha ))&=\mathscr {P}_f(\alpha )\vee \mathscr {P}_{\gamma _X}(\Box _X(\mathscr {P}_f(\alpha )))\\&=\mathscr {P}_f(\alpha )\vee \mathscr {P}_{\gamma _X}(\mathscr {P}_{\mathscr {F}(f)}(\Box _Y(\alpha )))\\&=\mathscr {P}_f(\alpha )\vee \mathscr {P}_f(\mathscr {P}_{\gamma _Y}(\Box _Y(\alpha )))\\&= \mathscr {P}_f(\alpha \vee \mathscr {P}_{\gamma _Y}(\Box _Y(\alpha )))\\&=\mathscr {P}_f(\diam {Y}(\alpha )) \end {align*} \par \par \item By hypothesis: \begin {align*} \alpha &\leq \bigwedge _{\beta \in \mathcal {N}_{\gamma _X}(\alpha )}\mathscr {P}_{\gamma _X}(\Box _X(\beta ))\\&= \mathscr {P}_{\gamma _X}(\bigwedge _{\beta \in \mathcal {N}_{\gamma _X}(\alpha )}\Box _X(\beta ))\\&= \mathscr {P}_{\gamma _X}(\Box _X(\bigwedge _{\beta \in \mathcal {N}_{\gamma _X}(\alpha )}\beta ))\\&=\mathscr {P}_{\gamma _X}(\Box _X(\mathsf {s}_{\gamma _X}(\alpha ))) \end {align*} \par \item The inequality $\alpha \leq \scat {X}(\alpha )$ follows at once, if $\alpha \leq \beta $ we have $\mathscr {P}_{\gamma _{X}}(\Box _X(\alpha ))$ as in the first point but this implies that $\mathcal {N}_{\gamma _X}(\beta )\subset \mathcal {N}_{\gamma _X}(\alpha )$. Hence, $\bigwedge _{\theta \in \mathcal {N}_{\gamma _X}(\alpha )}\theta \leq \bigwedge _{\theta \in \mathcal {N}_{\gamma _X}(\beta )}\theta $, from which we deduce the monotonicity of $\scat {X}$. Let now $f:X\rightarrow Y$ be an arrow such that \begin {center} \begin {tikzpicture} \node (A)at (0,0) {$X$}; \node (B)at (3,0) {$Y$}; \node (C)at (0,-1.5) {$\mathscr {F}(X)$}; \node (D)at (3,-1.5) {$\mathscr {F}(Y)$}; \draw [->](A)--(C) node[pos=0.5, left]{$\gamma _X$}; \draw [->](B)--(D) node[pos=0.5, right]{$\gamma _Y$}; \draw [->](A)--(B) node[pos=0.5, above]{$f$}; \draw [->](C)--(D) node[pos=0.5, below]{$\mathscr {F}(f)$}; \end {tikzpicture} \end {center} commutes, and notice that for all $\theta \in \mathcal {N}_Y(\alpha )$ then \begin {align*} \mathscr {P}_f(\alpha )&\leq \mathscr {P}_f(\mathscr {P}_{\gamma _Y}(\Box _Y(\theta ))) =\mathscr {P}_{\gamma _X}(\mathscr {P}_{\mathscr {F}(f)}(\Box _Y(\theta ))) =\mathscr {P}_{\gamma _X}(\Box _X(\mathscr {P}_f(\theta ))) \end {align*} hence $\mathscr {P}_f(\theta )\in \mathcal {N}_X(\mathscr {P}_f(\alpha ))$ and thus \begin {align*} \scat {X}(\mathscr {P}_f(\alpha ))& = \mathscr {P}_f(\alpha )\vee \mathsf {s}_{\gamma _X}(\mathscr {P}_f(\alpha ))=\mathscr {P}_f(\alpha )\vee \bigwedge _{\beta \in \mathcal {N}_X(\mathscr {P}_f(\alpha ))}\beta \\&\leq \mathscr {P}_f(\alpha )\vee \bigwedge _{\beta \in \mathcal {N}_X(\mathscr {P}_f(\alpha ))}\beta \\&\leq \mathscr {P}_f(\alpha )\vee \bigwedge _{\beta \in \mathcal {N}_Y(\alpha )}\mathscr {P}_f(\beta )\\&\leq \mathscr {P}_f(\alpha )\vee \mathscr {P}_f(\bigwedge _{\beta \in \mathcal {N}_Y(\alpha )}\beta )\\&=\mathscr {P}_f(\alpha \vee \mathsf {s}_{\gamma _Y}(\alpha )) =\mathscr {P}_f(\scat {Y}(\alpha )) \end {align*} and we are done. \qedhere \end {enumerate}\end{proof}
\label{proofsection:prAtEndxi}\begin{proof}[Proof of \autoref{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}Associativity of composition and the fact that $(x_1,...,x_n)$ is the identity for $[x_i:\sigma _i]_{i=1}^n$ follows from a straightforward computation. The empty context is clearly terminal while, given two contexts $\Gamma :=[x_i:\sigma _i]_{i=1}^n$ and $\Delta =[y_i:\tau _i]_{i=1}^m$ we can take their concatenation as a product $\Gamma \times \Delta $, the universal property follows immediately.\qedhere \end{proof}
\label{proofsection:prAtEndxiii}\begin{proof}[Proof of \autoref{thm:prAtEndxiii}]\phantomsection\label{proof:prAtEndxiii}Cfr. \cite {jacobs1999categorical}, proposition $2.3.2$. The existence of finite product is clear, let's show the closedness. Projecting and evaluating we have a sequent $w:(\sigma \rightarrow \tau )\times \sigma \vdash \pi _{\sigma \rightarrow \tau }(w)(\pi _\sigma (w)):\tau $, let $ev_\sigma $ be the class of $\pi _{\sigma \rightarrow \tau }(x)(\pi _\sigma (x))$ in $\term {(\sigma \rightarrow \tau ) \times \sigma }{\tau }$ and let's show its universality. Let $\rho $ be another type and $[M]\in \term {\rho \times \sigma }{\tau }$ then we must have a sequent $z:\rho \times \sigma \vdash M:\tau $ and, weakening, we can derive \begin {gather*} \inferrule *{\inferrule *{x:\rho , y:\sigma , z:\rho \times \sigma \vdash M:\tau \\x:\rho , y:\sigma \vdash (x,y):\rho \times \sigma } {x:\rho , y:\sigma \vdash M[(x,y)|z]: \tau }} {x:\rho \vdash \lambda y:\sigma .M[(x,y)|z]:\sigma \rightarrow \tau } \end {gather*} Let's define \begin {equation*} \Lambda ([M]):=[\lambda y:\sigma .M[(x,y)|z]\in \term {\rho }{\sigma \rightarrow \tau } \end {equation*} Computing we have \begin {align*} ev_{\sigma }\circ ( \Lambda ([M])\times 1_{\sigma })&=[\pi _{\sigma \rightarrow \tau }(w)(\pi _\sigma (w))[( (\lambda y:\sigma .M[(x,y)|z])[p_\rho (z)|x],p_\sigma (z))|w]]\\&=[(\lambda y:\sigma .M[(p_\rho (z),y)|z])(p_\sigma (z))]\\&=[M[(p_\rho (z),p_\sigma (z))|z]]\\&=[M] \end {align*} For uniqueness it's enough to notice that for any $[N]\in \term {\rho }{\sigma \rightarrow \tau }$: \begin {align*} \Lambda (ev_{\sigma }\circ ([N]\times 1_\sigma ))&=[\lambda y:\sigma .\pi _{\sigma \rightarrow \tau }(w)(\pi _\sigma (w))[(N,y)|w] ]\\&=[\lambda y:\sigma .N(y)]=[N] \qedhere \end {align*}\end{proof}
\label{proofsection:prAtEndxiv}\begin{proof}[Proof of \autoref{thm:prAtEndxiv}]\phantomsection\label{proof:prAtEndxiv}\begin {enumerate} \item The type formation rules and for $\propo $ tell us that $\term {-}{\propo }$ is a functor $\hoclass {\Sigma }^{op}\rightarrow \catname {HA}$ in which the closure operator is given by \begin {align*} \mathfrak {c}_\Sigma : \term {\sigma }{\propo } &\rightarrow \term {\sigma }{\propo }\\ [\phi ] &\mapsto [\mathcal {C}(\phi )] \end {align*} The fibered equality is given by the sequent \begin {gather*} (M,N):\sigma \times \sigma \vdash M=_\sigma N :\propo \end {gather*} Now notice that the rules of derivation tell us that \begin {align*} \term {\sigma \times \tau }{\propo } &\rightarrow \term {\sigma }{\propo }\\ \phi &\mapsto \exists _{x:\tau }(\phi ) \\[1ex] \term {\sigma \times \tau }{\propo } &\rightarrow \term {\sigma }{\propo }\\ \phi &\mapsto \forall _{x:\tau }(\phi ) \end {align*} are the left and right adjoint to \begin {align*} \term {\pi _\sigma }{\propo }:\term {\sigma }{\propo } &\rightarrow \term {\sigma \times \tau }{\propo }\\ \phi &\mapsto \phi \circ \pi _{\sigma } \end {align*} and that Frobenius reciprocity and the Beck-Chevalley condition hold, and so we can conclude. \item This follows immediately by the rules for conjunction. \qedhere \end {enumerate}\end{proof}
\label{proofsection:prAtEndxv}\begin{proof}[Proof of \autoref{thm:prAtEndxv}]\phantomsection\label{proof:prAtEndxv}Monotonicity and inflationarity comes at once, take an arrow $f:C\rightarrow D$, for any $\alpha \in \mathscr {P}(D)$ we have: \begin {align*} \exists _f(\reach {C}(\mathscr {P}_f(\varphi )))&=\exists _f(\mathscr {P}_f(\varphi ))\vee \bigvee _{p\in \catname {C}(I,C)}\exists _f(\exists _p(\uparrow \mathscr {P}_p(\varphi ))) \\&=\exists _f(\mathscr {P}_f(\varphi ))\vee \bigvee _{p\in \catname {C}(I,C)}\exists _f(\exists _{p}(\exists _{\pi _2}(\rho \wedge \mathscr {P}_{\pi _1}(\mathscr {P}_{p}(\mathscr {P}_{f}(\varphi ))))))\\&\leq \varphi \vee \bigvee _{p\in \catname {C}(I,C)} \exists _{f\circ p}(\exists _{p}(\exists _{\pi _2}(\rho \wedge \mathscr {P}_{\pi _1}(\mathscr {P}_{f\circ p}(\varphi ))))\\&\leq \varphi \vee \bigvee _{q\in \catname {C}(I,D)} \exists _{q}(\exists _{\pi _2}(\rho \wedge \mathscr {P}_{\pi _1}(\mathscr {P}_{q}(\varphi ))))\\&=\varphi \vee \bigvee _{q\in \catname {C}(I,D)}\exists _q(\uparrow \mathscr {P}_q(\varphi )) \\&=\reach {D}(\varphi ) \end {align*} Groundedness is immediate; suppose now that $\mathscr {P}$ is an hyperdoctrine, then $\mathscr {P}_f$ commutes with suprema for any arrow $f$ and, since $\mathscr {P}(C)$ is an Heyting algebra, infima distribute over them, so: \begin {align*} \reach {C}(\bigvee _{k\in K}\varphi _k)&= (\bigvee _{k\in K}\varphi _K )\vee \bigvee _{p\in \catname {C}(I,C)} \exists _{p}(\exists _{\pi _1}(\rho \wedge \mathscr {P}_{\pi _2}(\mathscr {P}_p(\bigvee _{k\in K}\varphi _k))))\\&=(\bigvee _{k\in K}\varphi _k)\vee \bigvee _{p\in \catname {C}(I,C)}\bigvee _{k\in K}\exists _{p}(\exists _{\pi _1}(\rho \wedge \mathscr {P}_{\pi _2}(\varphi _k)))\\&=\bigvee _{k\in K}(\varphi _k\vee \bigvee _{p\in \catname {C}(I,C)}\exists _{p}(\exists _{\pi _1}(\rho \wedge \mathscr {P}_{\pi _2}(\varphi _k))))\\&= \bigvee _{k\in K} \reach {C}(\varphi _k) \qedhere \end {align*}\end{proof}
\label{proofsection:prAtEndxvi}\begin{proof}[Proof of \autoref{thm:prAtEndxvi}]\phantomsection\label{proof:prAtEndxvi}\begin {enumerate} \item By continuity we have \begin {align*} \mathfrak {c}_I(\mathscr {P}_p(\alpha ))\wedge \mathscr {P}_p(\neg \alpha )&\leq \mathscr {P}_p(\mathfrak {c}_C(\alpha )) \wedge \mathscr {P}_p(\neg \alpha )\\&\leq \mathscr {P}_p(\mathfrak {c}_C(\alpha )\wedge \neg \alpha )\\&\leq \mathscr {P}_p(\psi ) \end {align*} By hypothesis, \begin {align*} \mathfrak {c}_I(\mathscr {P}_p(\alpha ))\wedge \mathscr {P}_p(\neg \alpha )&\leq \uparrow \mathscr {P}_p(\alpha )\\&\leq \mathscr {P}_p(\phi ) \end {align*} and \begin {align*} \mathfrak {c}_I(\mathscr {P}_p(\alpha ))\wedge \mathscr {P}_p(\neg \alpha )&=\mathfrak {c}_I(\mathscr {P}_p(\alpha ))\wedge \mathscr {P}_p(\neg \alpha )\wedge \top \\&=(\mathfrak {c}_I(\mathscr {P}_p(\alpha ))\wedge \mathscr {P}_p(\neg \alpha )\wedge \mathscr {P}_{p}(\phi ) )\vee (\mathfrak {c}_I(\mathscr {P}_p(\alpha ))\wedge \mathscr {P}_p(\neg \alpha )\wedge \mathscr {P}_p(\neg \phi ))\\&\leq \downarrow \mathscr {P}_p(\neg \phi ) \end {align*} hence, since $p\in \er {C}{\phi }{\psi }$: \begin {align*} \mathfrak {c}_I(\mathscr {P}_p(\alpha ))\wedge \mathscr {P}_p(\neg \alpha )&\leq \uparrow \mathscr {P}_p(\phi )\wedge \downarrow \mathscr {P}_p(\neg \phi )\wedge \mathscr {P}_p(\psi ) = \bot \end {align*} and we conclude by connectedness. \item By the previous point $\mathscr {P}_p(\alpha )=\bot $ for any $p\in \er {C}{\phi }{\psi }$ so $\mathscr {P}_p(\neg \alpha )=\top $ that implies $\alpha \leq \neg \exists _p(\top )$ from which the thesis follows. \qedhere \end {enumerate}\end{proof}

